Can NR-V2X Sidelink support A2A links?

In the context of 5G, 3GPP introduced New Radio vehicle to everything (NR-V2X) for direct vehicle-to-vehicle communication. However, starting from Release 18 the focus of the standard has been expanded from vehicles to any device and use case that can benefit from direct communication. In 3GPP terminology, the standard is now referred to simply as Sidelink communication. This standard allows direct communication between devices based on synchronous resource scheduling. Users can rely on controlled scheduling when in network coverage or, in the absence of coverage, autonomously select resources for transmission via a distributed resource allocation mechanism. Focusing on the autonomous resource allocation, this paper investigates the possibility of applying Release 18 Sidelink communication to Air-to-Air (A2A) links between airborne entities. The paper outlines the main challenges and required modifications to adapt the current standard for longer links in the order of kilometres. The analysis identifies the propagation delay as a critical limitation. Communications at distances over 42.4 km require a restriction of the user's transmitting opportunities. However, sidelink communication remains feasible for distances below this threshold without modifications to the standard.

==> TableSettings.tex <==
\begin{table}[!t]
\caption{Main simulation settings. 
\vspace{-2mm}
\label{Tab:Settings-ap}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{4cm}p{3.9cm}}
\hline \hline
%\textbf{Common parameters (Symbol)} & \textbf{Value} \\  
%\hline
\emph{\textbf{Scenario}} & \\
%Simulated time ($\Tsim$) & 90 s \\
%Position of vehicles & Highway \\
%\textbf{\textit{Scenario}} & \\
Road layout & Octagon configuration \\
Density & 8 nodes \\
Average speed & $130$ km/h \\ \hline
\emph{\textbf{Power and propagation}} & \\
Channels & ITS bands at 5.9 GHz \\
Bandwidth & 1000 MHz \\
Transmission power & 40~dBm \\
Antenna gain (tx and rx)  & 12 dBi \\
Noise figure & 8~dB \\
Propagation model & Free space \\
%Shadowing & Var. 3 dB, decorr. dist. 25~m \\
%Fast fading & Highway LOS fading model \\ 
\hline
\emph{\textbf{Data traffic}}& \\
%Aperiodic packet generation & 50 ms fixed + 50 ms random\\ 
GNSS positioning generation
& 10 Bytes every 500 ms\\
Video streaming generation & 4500~bytes every 4 ms\\
Advanced driving generation & 20~bytes every 20 ms\\
\hline
\emph{\textbf{Access layer (NR-V2X)}} & \\
%SI cancellation factor & -110 dB \\
%Collision detection threshold & Optimized per each density \\
MCS & 15 (16QAM, $R_\text{c}=0.6$) \\
SINR threshold &  16.6 dB \cite{todisco2021performance} \\
Subchannel size & \mbox{10 PRB} \\%physical resource blocks} \\
Number of subchannels & 13 \\
SCS & 60 kHz \\
Keep probability & 0 \\
SB-SPS RSRP sensing threshold & -$126$~dBm  \\%-110, -120, -126~dBm \\
Min. time for the allocation, $T_1$ & $1$~ms \\
Max. time for the allocation, $T_2$  & $4$~ms\\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}

